Extended Field Theories as higher Kaluza-Klein theories

Extended Field Theories include Double Field Theory (DFT) and Exceptional Field Theory, which are respectively the T- and U-duality covariant formulations of the supergravity limit of String Theory and M-theory. Extended Field Theories do not live on spacetime, but on an extended spacetime, locally modelled on the space underlying the fundamental representation of the duality group. Despite its importance in M-theory, however, the global understanding of Extended Field Theories is still an open problem. In this thesis we propose a global geometric formulation of Extended Field Theory. Recall that ordinary Kaluza-Klein theory unifies a metric with a gauge field on a principal bundle. We propose a generalisation of the Kaluza-Klein principle which unifies a metric and a higher gauge field on a principal infinity-bundle. This is achieved by introducing an atlas for the principal infinity-bundle, whose local charts can be naturally identified with the ones of Extended Field Theory. Thus, DFT is interpreted as a higher Kaluza-Klein theory set on the total space of a bundle gerbe underlying Kalb-Ramond field. As first application, we define the higher Kaluza-Klein monopole by naturally generalising the ordinary Gross-Perry monopole. Then we show that this monopole is exactly the NS5-brane of String Theory. Secondly, we show that our higher geometric formulation gives automatically rise to global abelian T-duality and global Poisson-Lie T-duality. In particular, we globally recover the abelian T-fold and we define the notion of Poisson-Lie T-fold. Crucially, we will investigate the global geometric formulation of tensor hierarchies and gauged supergravity. In particular, we will provide a global formulation of generalised Scherk-Schwarz reductions and we will discuss their global non-geometric properties. Finally, we explore the T-duality covariant geometric quantisation of DFT.

==> text/notation.tex <==
% First parameter can be changed eg to "Glossary" or something.
% Second parameter is the max length of bold terms.
\begin{mclistof}{Notation}{3.2cm}

\subsection*{Higher geometry}

\item[$\mathbf{G},\mathbf{H},\mathbf{K}\dots$] Categories, $(\infty,1)$-categories

\item[$\mathscr{G},\mathscr{H},\mathscr{K}\dots$] Smooth stacks

\item[$G,H,K,\dots$] Lie groups, Lie $\infty$-groups

\item[$\mathfrak{g},\mathfrak{h},\mathfrak{k},\dots$] Lie algebras, $L_\infty$-algebras

\item[$\mu,\nu,\lambda,\dots$] One- or two-dimensional, referring in this thesis to spatial dimensions in an image

\item[$(\alpha),(\beta),(\gamma),\dots$]  Indices of the patches of a cover

\subsection*{Supergeometry}

\item[$\upalpha,\upbeta,\upgamma,\dots$]  Indices of the patches of a cover

\item[$\mathsf{m},\mathsf{n},\mathsf{l},\dots$]  Indices of the patches of a cover

\item[$\mathsf{a},\mathsf{b},\mathsf{c},\dots$]  Indices of the patches of a cover

\subsection*{Double Field Theory}

\item[$\mathbbvar{x}^M=(x^\mu,\widetilde{x}_\mu)$] One- or two-dimensional, referring in this thesis to spatial dimensions in an image

\subsection*{Cohomology theory}

\item[$H^\bullet(-,\mathbb{Z})$]  Indices of the patches of a cover

\item[$H^\bullet(-,G)$]  Non-abelian cohomology

\item[$H^\bullet_\mathrm{dR}(-)$] de Rham cohomology

\item[$\mathbf{H}(-,-)$] Cocycle $\infty$-groupoid

\subsection*{Numbers}

\item[$\mathbb{N}^+$] Positive integer numbers

\item[$\mathbb{R}^+$] Positive real numbers

\end{mclistof} 

